Updated observing scenarios and multi-messenger implications for the International Gravitational-wave Network's O4 and O5

An advanced LIGO and Virgo's third observing run brought another binary neutron star merger (BNS) and the first neutron-star black hole mergers. While no confirmed kilonovae were identified in conjunction with any of these events, continued improvements of analyses surrounding GW170817 allow us to project constraints on the Hubble Constant ($H_0$), the Galactic enrichment from $r$-process nucleosynthesis, and ultra-dense matter possible from forthcoming events. Here, we describe the expected constraints based on the latest expected event rates from the international gravitational-wave network (IGWN) and analyses of GW170817. We show the expected detection rate of gravitational waves and their counterparts, as well as how sensitive potential constraints are to the observed numbers of counterparts. We intend this analysis as support for the community when creating scientifically driven electromagnetic follow-up proposals. During the next observing run O4, we predict an annual detection rate of electromagnetic counterparts from BNS of $0.43^{+0.58}_{-0.26}$ ($1.97^{+2.68}_{-1.2}$) for the Zwicky Transient Facility (Rubin Observatory).

==> EOS.tex <==
\begin{abstract}

Advanced LIGO and Virgo's third observing run brought another binary neutron star merger (BNS) and the first neutron-star black-hole (NSBH) mergers. 
While no confirmed counterpart was identified to any of these events, continued improvements of analyses surrounding GW170817 allow us to project the Hubble Constant ($H_0$) and neutron star equation of state constraints possible from forthcoming events.
Here, we describe the expected constraints based on the latest expected event rates and analyses of GW170817.
We show the expected detection rate of gravitational-wave counterparts, and how sensitive these constraints are to the observed numbers of counterparts.
Analyses of this kind are useful for scientific driven electromagnetic follow-up proposals.
\end{abstract}


\section{Introduction}
In our work, we will study how tight constraints on $H_0$ and the equation of state of neutron stars (EoS) will be in future observing runs, including the number of detections required to be competitive with other methods. 
We will present quantitative studies on the following  topics based on our simulation sets:
\begin{itemize}
    \item EoS constraints (represented as constraints on the radius for a 1.4M$_{sun}$ NS)
    \item H$_{0}$ constraints
    \item studying the prompt collapse of a NS merger into a black hole
    \item empirical measurement of merger accretion disk fraction producing a KN
    \item joint EM+GW binary inclination angle constraints, therefore improving H$_0$ measurement
\end{itemize}
In Sec.~\ref{sec:}, we will  joint EM and GW posteriors to constraint EoS and improve $H_0$ measurement. In Sec.~\ref{sec:conclusion}, we present our conclusions and implications for future follow-up strategies.


\section{GW EM conterpart}
\subsection{EoS constraints}

\begin{figure*}
    \includegraphics[width=3.5in]{figures/R14_trend_GW_EM_ZTF.pdf}
    \includegraphics[width=3.5in]{figures/R14_trend_GW_EM_Gemini.pdf}
    \caption{
    $\sigma_{R_{1.4M\odot}}$ estimate for our sample. We show our combined measurement (green violin), gravitational-wave (blue) and electromagnetic measurements (orange). The top and bottom rows are the BNS and NSBH set respectively, both for the full sample (left) and detections only (right). The limit from GW170817 and its electromagnetic counterparts is shown in dashed cyan.}
    \label{fig:R14}
\end{figure*}

Taking the distribution of all detections, we present equation of state constraints based on the expected binary neutron star detections during O4 in Figure~\ref{fig:R14}.
Taking the median residual for the analyses, we demonstrate that we can constrain the radius of a 1.4 $M_\odot$ neutron star to $\sigma_{R_{1.4M\odot}} = 0.4 \mathrm{km}$ and $\sigma_{R_{1.4M\odot}} = 0.2 \mathrm{km}$ for the electromagnetic analysis, $\sigma_{R_{1.4M\odot}} = 0.1 \mathrm{km}$ and $\sigma_{R_{1.4M\odot}} = 0.05 \mathrm{km}$ for the gravitational-wave analysis, and $\sigma_{R_{1.4M\odot}} = 0.1 \mathrm{km}$ and $\sigma_{R_{1.4M\odot}} = 0.04 \mathrm{km}$ for the combined analysis for 10 and 50 detections respectively. This measurement will place strong constraints on the cold supranuclear EOS. 

\subsection{$H_0$ constraints}

\begin{figure*}
    \includegraphics[width=3.5in]{figures/H0_trend_GW_EM_ZTF.pdf}
    \includegraphics[width=3.5in]{figures/H0_trend_GW_EM_Gemini.pdf}
    \label{fig:H0}
    \caption{
    $\sigma_{H_0}$ estimate from the same samples. The top and bottom rows are the BNS and NSBH set respectively, both for the full sample (left) and detections only (right). We show our combined measurement (green violin), gravitational-wave (blue) and electromagnetic measurements (orange). The top and bottom rows are the BNS and NSBH set respectively, both for the full sample (left) and detections only (right). In addition, we show the Planck measurement of the Cosmic Microwave Background~\cite{Ade:2015xua} (Planck CMB, purple) and the Hubble measurement via type-Ia supernovae~\cite{Riess:2016jrr} (SNIa, blue). All uncertainty refer to a $1\sigma$ measurement.}
\end{figure*}

To determine the posterior distribution for $H_0$, we take a basic cosmology model appropriate for a nearby event $D = \frac{z \times c}{H_0}$.
We perform three analyses. The first uses the BAYESTAR
distance estimate along the line of sight of the transient to approximate the gravitational-wave distance posterior. The second uses the distance inferred from the kilonova analysis. The third uses a combined analysis, multiplying the gravitational-wave and electromagnetic distance probabilities.
In Figure~\ref{fig:H0}, we show the expected $H_0$ constraints based on that detected simulation set. We also constrain $H_0$ to $\sigma_{H_0} = 3.4$\,$\mathrm{km}$ $\mathrm{s}^{-1}$ $\mathrm{Mpc}^{-1}$ and $\sigma_{H_0} = 2.0$\,$\mathrm{km}$ $\mathrm{s}^{-1}$ $\mathrm{Mpc}^{-1}$ for the electromagnetic analysis, $\sigma_{H_0} = 3.5$\,$\mathrm{km}$ $\mathrm{s}^{-1}$ $\mathrm{Mpc}^{-1}$ and $\sigma_{H_0} = 2.3$\,$\mathrm{km}$ $\mathrm{s}^{-1}$ $\mathrm{Mpc}^{-1}$ for the gravitational-wave analysis, and $\sigma_{H_0} = 3.0$\,$\mathrm{km}$ $\mathrm{s}^{-1}$ $\mathrm{Mpc}^{-1}$ and $\sigma_{H_0} = 1.7$\,$\mathrm{km}$ $\mathrm{s}^{-1}$ $\mathrm{Mpc}^{-1}$ for the combined analysis for 10 and 50 events respectively. This projection improves on what has been achieved so far with GW170817 and its electromagnetic counterparts by about a factor of 3 and is competitive with the the Planck measurement of the Cosmic Microwave Background~\cite{Ade:2015xua} and type-Ia supernovae~\cite{Riess:2016jrr}.
    

5) joint EM+GW inclination angle constraints (also improvement of H0)    



\section{Conclusion}
\label{sec:conclusion}    

In this paper, we have performed an end-to-end gravitational-wave survey simulation for O4 and O5 follow-up of binary neutron star and neutron-star black-hole mergers.
Using a distance threshold of 300\,Mpc, we simulate follow-up of relatively nearby events for ZTF follow-up.
Based on the gravitational-wave and kilonova posteriors from these analyses, we simulate the potential $H_0$ and EOS constraints.

With the simulation study performed above, we can summarize our conclusions and implications for future gravitational-wave follow-ups as follows:
\begin{description}[font=$\bullet$~\normalfont\scshape]
\item [\textcolor{red}{Event selection}] During O4 and beyond, there will be many more events than are reasonable to follow-up. Unsurprisingly, the objects that are best to follow-up are the best localized and near-by \citep{ChHo2016}. 
% How near-by 
Proximity is an especially important consideration for the neutron-star black-hole mergers, given their large expected distances and faint intrinsic luminosities. 
\item [\textcolor{red}{Neutron star EOS}] The gravitational-wave contribution dominates under the assumptions in this document, but again, high SNR, near-by events dominate the sensitivity improvement. A few well-localized near-by events are worth much more than many far away, poorly localized events.
\item [\textcolor{red}{$H_0$}] Most events contribute equally, especially as relative uncertainty due to virial velocities decreases as distance increases.
\end{description}    

==> get-out-mass-gap.tex <==

we determine the range R or the maximum sensitive distance (radius of an Euclidean sphere) for each of our samples. This computed range allows us to assign each of our samples uniformly in a sensitive space-time volume (i.e.\ the volume comoving by a factor (1 + z), due to the expansion of the Universe), $ \frac{4}{3}\pi \text{R}^3 = \text{V}_z$, with $\text{V}_z$. Inside this volume, we draw samples uniformly and isotropically, a distribution of distances and sky locations joined to our CBCs and  using cosmological parameters in.

\subsection{Getting out of the mass gap }

\label{subsec:mass-gap}
The analysis of the data from all detections of gravitational waves carried out by the LIGO-Virgo-KAGRA (LVK) collaboration from Run O1 to Run O3a gives a stiffening of the power law describing NSs and low-mass BHs with a confidence of 99.3$\%$ below ${2.4}_{-0.5}^{+0.5}\,\,\text{M}_{\odot }$ \citep{Farah_2022}.  From these data we can note : \\
i) The second  mass ($\text{m}_2 = {2.59}_{-0.09}^{+0.08}\,\,\text{M}_{\odot }$) of  GW190814 event is so far identified as the most massive of all the NS astrophysical populations \citep{Abbott_2020}. \\
ii) While the lower limit of a black hole is one of the components of GW190917\_114630, lying below $3\,\text{M}_{\odot }$ and thus as having a high probability of being a NS instead of a BH.\\ 
Considering the EoS as well as the recent astrophysical observations, in particular GW170817, the mass limit of a neutron star without any rotation cannot exceed the Tolman-Oppenheimer-Volkoff (TOV) mass $\text{M}_{\text{max, TOV}} \approx 2.2 - 2.5\,\, \text{M}_\odot$, 
and backed by \citep{PhysRevD.104.063003, PhysRevD.97.021501, PhysRevD.100.023015, 2017ApJ...850L..19M} $\approx 2 - 2.5\,\, \text{M}_\odot$. \\
iii) At the same time, analyses of the mass distributions of BHs based on X-ray binary systems \citep{_zel_2016, 2011ApJ...741..103F}  suggest that the minimum mass of a BH is  $5\,\, \text{M}_\odot$. In this case the upper-limit(NS) $\ne$ lower-limit(BH) and there exists a mass gap.\\
iv) Work by \citealt{2020ApJ...899L...8F} on GWTC-1 events and \citealt{2021ApJ...913L...7A} on GWTC-2 showed that a single power law cannot fit the mass distribution of BBHs and BNSs.\\


